TRIDENT: The Nonlinear Trilogy for Implicit Neural Representations

Implicit neural representations (INRs) have garnered significant interest recently for their ability to model complex, high-dimensional data without explicit parameterisation. In this work, we introduce TRIDENT, a novel function for implicit neural representations characterised by a trilogy of nonlinearities. Firstly, it is designed to represent high-order features through order compactness. Secondly, TRIDENT efficiently captures frequency information, a feature called frequency compactness. Thirdly, it has the capability to represent signals or images such that most of its energy is concentrated in a limited spatial region, denoting spatial compactness. We demonstrated through extensive experiments on various inverse problems that our proposed function outperforms existing implicit neural representation functions.

==> tab/SISR_summary.tex <==
\renewcommand{\arraystretch}{1.6}
\begin{table*}[!htp]
\scriptsize
\centering
\tabcolsep=0.06cm
% \hskip-6.5em
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
Method(PSNR)& Monarch   &baby  &Zebra &Pepper&average\\\hline
SIREN       & 24.21     &28.99 &23.04 &26.63 & 25.72\\\hline
WIRE        & 25.18     &30.35 &23.07 &27.21 &26.45\\\hline
FourierNet  &           &      &      &      &       \\\hline
OURS        & 25.34     &30.56 &23.26 &27.27 &26.61\\\hline
\end{tabular}
\caption{\label{tab:widgets}Table showing the 4x super-resolution result of Monarch, baby, zebra, pepper and the average PSNR from SIREN, WIRE, Fourier Feature Networks (FourierNet), and our proposed network in Single image Super-resolution .}
\label{sisrtable}
\end{table*}

==> tab/audiotable.tex <==
\renewcommand{\arraystretch}{1.6}
\begin{table}[!htp]
\scriptsize
\centering
\tabcolsep=0.06cm
% \hskip-6.5em
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Method & Old-friends& Music \\\hline
SIREN &0.000235& \\\hline
WIRE &0.011515&0.023802  \\\hline
FourierNet &        &\\\hline
OURS       &0.000157&0.000779\\\hline
\end{tabular}
\caption{\label{tab:widgets}Table showing experiments of SIREN, WIRE, Fourier Feature Networks (FourierNet), and our proposed network.}
\end{table}

==> tab/formulatable.tex <==
% \begin{table*}[t!]
% %\scriptsize
% \centering
% \tabcolsep=0.06cm
% % \hskip-6.5em
% \resizebox{1\textwidth}{!}{%
% \begin{tabular}{|l|c|c|c|c|}
% \hline
% \textsc{Method} & Formula(in real context)  & Compactness&Even/Odd Features \\\hline
% SIREN~\cite{sitzmann2020implicit} & $\sin{(Wx+b)}$& Frequency&Odd  \\\hline
% WIRE~\cite{saragadam2023wire} & $\exp{(i\omega_0 (Wx+b))} \exp{(-\| s_0 (Wx+b)\|^2)}$ & Frequency and Spatial&Even \\\hline

% TRIDENT & $\exp(-\|s_0\left[x, \cdots \cos \left(2 \pi \sigma^{j / m} \mathbf{x}\right), \sin \left(2 \pi \sigma^{j / m} \mathbf{x}  \right) \cdots \right]^{\mathrm{T}}\|^2)$&  Order, Spatial and Frequency&Odd and Even  \\\hline
% \end{tabular}
% }
% \label{tab:widgets}
% \caption{Table summarising the activation function and compactness properties of SIREN, WIRE, and our proposed network. \Angie{we will remove this table}}
% \end{table*}


\begin{table*}[]
\resizebox{1\textwidth}{!}{%
\begin{tabular}{lccc}
\hline
\multicolumn{1}{l|}{\textsc{Method}} & \multicolumn{1}{c|}{\textsc{Formula}} & \multicolumn{1}{c|}{\textsc{Compactness}} & \textsc{Even/Odd Features} \\ \hline
SIREN~\cite{sitzmann2020implicit}  & $\sin{(Wx+b)}$ & Frequency & Odd \\ \hline
WIRE~\cite{saragadam2023wire}  & $\exp{(i\omega_0 (Wx+b))} \exp{(-\| s_0 (Wx+b)\|^2)}$ & Frequency and Spatial & Even \\ \hline
\trident & $\exp(-\|s_0\left[x, \cdots \cos \left(2 \pi \sigma^{j / m} \mathbf{x}\right), \sin \left(2 \pi \sigma^{j / m} \mathbf{x}  \right) \cdots \right]^{\mathrm{T}}\|^2)$ & Order, Spatial and Frequency & Odd and Even \\ \hline
\end{tabular}
}

\caption{Table summarising the activation function and compactness properties of SIREN, WIRE, and our proposed network.}
\end{table*}
